Improved Diffusion-based Image Colorization via Piggybacked Models

Image colorization has been attracting the research interests of the community for decades. However, existing methods still struggle to provide satisfactory colorized results given grayscale images due to a lack of human-like global understanding of colors. Recently, large-scale Text-to-Image (T2I) models have been exploited to transfer the semantic information from the text prompts to the image domain, where text provides a global control for semantic objects in the image. In this work, we introduce a colorization model piggybacking on the existing powerful T2I diffusion model. Our key idea is to exploit the color prior knowledge in the pre-trained T2I diffusion model for realistic and diverse colorization. A diffusion guider is designed to incorporate the pre-trained weights of the latent diffusion model to output a latent color prior that conforms to the visual semantics of the grayscale input. A lightness-aware VQVAE will then generate the colorized result with pixel-perfect alignment to the given grayscale image. Our model can also achieve conditional colorization with additional inputs (e.g. user hints and texts). Extensive experiments show that our method achieves state-of-the-art performance in terms of perceptual quality.

==> graphs/domain_gap.tex <==
\captionsetup[subfigure]{labelformat=empty}
\def\myhighreswidth{0.15}
\def\myhighresoffset{0.00}
\centering
\begin{tabular}[c]{cccccc}
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/gt1.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/gray1.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/out1.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/outs1.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/dg1.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/dgs1.png}\end{subfigure}
        \\
        Ground Truth  & Grayscale Input & \multicolumn{2}{c}{Unconditional Colorization} & "pokemon" & "pikachu"
        \\
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/gt2.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/gray2.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/out2.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/outs2.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/dg2.png}\end{subfigure}
        &
        \begin{subfigure}[b]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/domain_gap/dgs2.png}\end{subfigure}\\
        Ground Truth  & Grayscale Input & \multicolumn{2}{c}{Unconditional Colorization} & "japanese cartoon" & "doraemon"
\end{tabular}

==> graphs/text_showcase2.tex <==
\captionsetup[subfigure]{labelformat=empty}
\def\myhighreswidth{0.22}
\def\myhighresoffset{0.0}
\centering
\begin{tabular}[c]{cccc}
\multirow{2}{*}{
\begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/warm_feeling_gray.jpg}
        \subcaption{Grayscale Input}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}
        }
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/warm_feeling_gt.jpg}
        \subcaption{Ground Truth}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/warm_feeling_ours.jpg}
        \subcaption{"warm feeling"}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/02cold.png}
        \subcaption{"cold feeling"}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}
        \\
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/02uncond.png}
        \subcaption{Unconditional colorization}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/02colorful.png}
        \subcaption{"colorful"}
        \end{subfigure}
        &
        \begin{subfigure}[c]{\myhighreswidth\textwidth}\includegraphics[width=\textwidth]{graphs/text_showcase/02old.png}
        \subcaption{"old photo"}
        \end{subfigure}\hspace{\myhighresoffset\textwidth}

\end{tabular}
